AI Incident Monitoring through a Public Health Lens

Artificial intelligence systems are now deployed at scale across sectors, accompanied by a growing number of real-world incidents ranging from misinformation and cybercrime to autonomous-system failures. Databases of AI incidents index these events, but they cannot measure ``risk'' (i.e., a joint measure of likelihood and severity) without additional data regarding the prevalence of risk-associated systems and their incident reporting rates. As a result, policymakers, companies, and the general public lack a means to weigh the benefits of AI against their in-context risks. Inspired by public-health processes, which presume noisy and incomplete disease surveillance, we identify six phases of incident emergence. We demonstrate the framework through a detailed case study of autonomous vehicles, whose mandatory reporting requirements produces reliable incident-rate ground truth expressed in distance traveled. The case study shows that an informed panel of domain experts (e.g., self-driving experts) can combine their domain expertise, incident data, and a collection of statistical and visualization tools to arrive at incident phase determinations serving public needs. We further demonstrate the approach with a deepfake incident case study and chart a path for future research in incident phase determination.

==> main_document/0_plain_language_summary.tex <==
\section*{Plain Language Summary}
\label{sec:0_plain_language_summary}

ABOVE MIGRATED

\noindent\rule{8cm}{0.4pt}

BELOW NOT MIGRATED

\toreview\

AI systems are now used in everyday settings-from cars and social media platforms to customer service tools and creative applications. As these systems spread, more incidents are reported in the news and in public databases: fraudulent deepfakes, unsafe autonomous vehicle behaviour, misleading recommendations, and many others. But these reports do not tell us, on their own, whether a type of AI harm is becoming more common, staying rare, or being brought under control. Reporting delays, media attention, and differences in how widely systems are used can all distort the picture.

In this paper, we introduce a practical way to make sense of this noisy evidence. Instead of counting incidents directly, we look at how a type of incident appears to move through a \emph{lifecycle}: from not yet observed, to rare, to rapidly increasing, to persistent (endemic), and in some cases to becoming rare again once mitigations take effect. To do this, we correct for known biases-for example, adjusting for how quickly incidents are reported, how widely a system is deployed, and how much media attention affects the likelihood that an incident is noticed.

We test this approach on two concrete examples: autonomous-vehicle crashes and deepfake harms. The results show that some harms fluctuate with deployment cycles, while others have undergone clear growth phases that simple incident counts would misrepresent.

This phase-based perspective helps policymakers, developers, and civil-society groups see where attention is most needed. It offers a clearer way to judge whether an AI-related risk is emerging, accelerating, stabilizing, or improving-even when the underlying data are incomplete.

\subsection*{What We Did}

Our aim was to develop a principled and interpretable way to understand how different types of AI-related harms emerge, accelerate, stabilize, or decline over time, despite the fact that existing incident datasets are noisy, incomplete, and shaped by media dynamics. To do this, we adapted methods from public-health surveillance-where similar challenges arise due to under-reporting, reporting delays, and heterogeneous observability-and applied them to AI incident data collected from the AI Incident Database (AIID) and related sources.

We built a modelling pipeline with four core components:

\begin{enumerate}
    \item \textbf{Reporting-delay correction.} Incident reports often appear weeks or months after the underlying event. We estimated a log-normal reporting-delay distribution using timestamp fields in AIID and applied nowcasting and backcasting procedures to reconstruct an event-time series for each incident class.

    \item \textbf{Exposure normalisation.} Raw incident counts rise mechanically as AI systems become more widely deployed. To separate scale effects from genuine changes in risk, we normalised by domain-specific exposure proxies: autonomous-vehicle miles  driven from California DMV records for AV incidents, and a cumulative, diffusion-style synthetic exposure curve for deepfakes, where direct usage data are unavailable.

    \item \textbf{Media adjustment.} For categories with heavy media amplification-such as deepfakes-we introduced media covariates (e.g., Google Trends indices) into Negative Binomial models to adjust observed counts for attention-driven fluctuations.

    \item \textbf{Latent phase inference.} Using the cleaned, exposure-adjusted series, we inferred latent risk phases through regime-switching and segmentation methods. These included Hidden Markov Models (for oscillatory or multi-regime systems), PELT changepoint detection (for structural transitions), K-means clustering (as an independent validity check), and trend estimation via Negative Binomial GLMs. Each model supports classification into six lifecycle phases: \textit{no evidenced occurrence, rare occurrence, rapid expansion, endemic unmitigated, endemic mitigated,} and \textit{rare mitigated}.
\end{enumerate}

To demonstrate the framework, we applied the full pipeline to two priority incident classes from the MIT AI Risk Repository taxonomy: \textbf{autonomous vehicles} and \textbf{deepfake-enabled harms}. These subdomains were selected because they have: (i) a clear mapping to specific system types, (ii) sufficient temporal coverage in AIID, and (iii) policy audiences for whom trajectory and phase information are decision-relevant.

All analyses were implemented using openly accessible data and are fully reproducible via the code repository linked in the abstract. The Appendices provide detailed model specifications, diagnostic checks, and sensitivity analyses.

\subsection*{What We Found}

Our empirical analysis shows that, once corrected for reporting delays, exposure growth, and media dynamics, AI incident trajectories reveal structured temporal patterns that are not visible in raw counts alone. These patterns differ substantially across incident domains, underscoring the need for phase-based interpretation rather than simple trend reading.

\paragraph{1. Raw incident counts are misleading without delay, exposure, and media correction.}
Across both case studies, naive counts overstated or understated underlying dynamics.  Reporting delays of 150--170 days suppressed recent events; exposure growth inflated  apparent risk in years of rapid system adoption; and media cycles produced short-lived visibility spikes that resembled risk surges. After adjustment, several apparent trends in the uncorrected data disappeared or reversed.

\paragraph{2. Autonomous-vehicle incidents exhibit oscillatory, multi-regime behavior.}
For autonomous vehicles, exposure-adjusted incident rates did not show sustained  acceleration. Instead, the Hidden Markov Model identified \textbf{recurrent transitions} between baseline, elevated, and high-risk states aligned with deployment expansions, system updates, and governance shocks. These “crisis–recovery” cycles reflect a domain where risk fluctuates as testing environments and operating conditions evolve. The stabilized plateaus indicate periods of \textit{endemic unmitigated} risk, while temporary declines following regulatory interventions correspond to \textit{endemic mitigated} phases.

\paragraph{3. Deepfake-enabled harms show a persistent upward trajectory that has not reversed.}
In contrast, deepfake incidents followed a \textbf{unidirectional growth path}. PELT changepoint detection revealed a marked structural shift around 2023, consistent with increased model accessibility, widespread diffusion of generative tools, and heightened social salience. Even after adjusting for media attention, the post-2023 period exhibited sustained elevation in the exposure-adjusted rate, indicative of a transition into \textit{rapid expansion} and subsequently \textit{endemic unmitigated} conditions. The Negative Binomial model confirmed that media effects significantly influence reporting but do not fully account for the underlying rise.

\paragraph{4. Phase classification produces a clearer and more actionable summary of risk.}
Across both domains, the six-phase framework provided an interpretable and governance- relevant summary of incident dynamics. The combination of risk level (standardised, exposure-adjusted rate) and trajectory (short-term slope) yielded consistent phase assignments across methods. Uncertainty was quantified using HMM state probabilities, confidence intervals on GLM trends, and sensitivity checks on changepoint penalties.

The resulting phase timelines reveal:
\begin{itemize}
    \item Long early periods of \textit{rare occurrence} for several harms;
    \item Identifiable moments of \textit{rapid expansion} linked to capability diffusion or deployment changes;
    \item Extended stretches of \textit{endemic unmitigated} conditions where harms persist at elevated levels; and
    \item Partial transitions into \textit{endemic mitigated} phases following regulatory or technical interventions.
\end{itemize}

\paragraph{5. Our phase model could serve as a foundation for governance-relevant monitoring.}
Because phase assignments update as new reports arrive, they offer a \textbf{dynamic map}
of how risks evolve. This enables:
\begin{itemize}
    \item Earlier detection of emerging or accelerating harms;
    \item Clearer interpretation of whether interventions are working;
    \item More proportionate allocation of oversight capacity; and
    \item A consistent basis for cross-domain comparison.
\end{itemize}

These findings demonstrate that, even with imperfect surveillance data, structured temporal regimes can be inferred and translated into practical signals for policymakers, regulators, AI developers, and civil-society stakeholders.

==> main_document/3_autonomous_vehicles.tex <==
Recognizing the aforementioned dataset issues, we now consider what phase determination we would make for an incident type where there are alternate sources of information providing strong ground truths. By comparing the incident determination with and without the strong ground truth, we can gain confidence in the capacity for human expert panels to arrive at similar determinations for incident types lacking ground truth.

We analyzed 75 Autonomous Vehicle (AV) incidents (565 reports) from July 2014 to February 2025 following the pipeline in Appendix~\ref{sub:a_data_processing_pipeline}. Table~\ref{tab:av_data_overview} summarizes data features for our AV case study, and domain-specific parameters are reported in Table~\ref{tab:av_model_parameters}.

\begin{table}[htbp]
\centering
\caption{Autonomous Vehicles: Data Overview.}
\label{tab:av_data_overview}
\begin{tabular}{lc}
\toprule
Feature & Autonomous Vehicles \\
\midrule
Unique incidents & 75 \\
Media reports & 565 \\
Observation period & Jul 2014 -- Feb 2025 \\
Months observed & 128 \\
Mean reporting delay (days) & 170 \\
Zero-incident months & 57.0\% \\
Exposure data source & CA DMV miles \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\caption{Autonomous Vehicles: Model Parameters.}
\label{tab:av_model_parameters}
\small
\begin{tabular}{lll}
\toprule
Model & Parameter & Value \\
\midrule
Delay model & $\mu$, $\sigma$ & 2.84, 2.59 \\
HMM & States & 6 \\
\gls*{pelt} & Penalty & 2.43 \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/fig4_aiid_vs_dmv_comparison.png}
    \caption{Monthly comparison of AIID-reported autonomous vehicle incidents (top) and California DMV official collision reports (bottom) for autonomous vehicles in the state, 2019--2025. While the AIID data includes autonomous car crashes outside the state of California, the strong reporting requirements for both miles traveled and incidents in the state provides a normalizer against which the number of incidents in the AIID can be compared.}
    \label{fig:aiid_v_dmv_comp}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/fig5_aiid_vs_dmv_normalized.png}
    \caption{Normalized comparison of AIID incidents and DMV collisions ($r = 0.12$). Both series are min-max scaled to [0, 1] for visual comparison.}
    \label{fig:aiid_v_dmv_norm}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/fig6_aiid_vs_dmv_scatter.png}
    \caption{Scatter plot of monthly AIID incident counts against DMV collision counts with linear fit ($r = 0.12$). The weak positive correlation reflects the fundamental mismatch between media-reported incidents and official collision records.}
    \label{fig:aiid_v_dmv_scatter}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/fig7_phase_agreement.png}
    \caption{Phase classification agreement between AIID-derived phases and DMV ground-truth phases. Top: AIID incidents colored by assigned phase. Middle: DMV collisions colored by assigned phase. Bottom: month-by-month agreement (green) or disagreement (red), with overall agreement of 14.1\%.}
    \label{fig:phase_agreement}
\end{figure}

The AIID data may have little correlation with the DMV ground truth as shown by Figure \ref{fig:aiid_v_dmv_norm}, but it is sufficient to arrive at a conclusion consistent with the ground truth data. We now examine the question of how effective a panel of human experts well-informed about the state of autonomous car deployments could utilize the AIID data to inform phase determinations in the absence of the ground truth DMV data.

% \todo{Expert panel results needed here. This section 
% requires input from domain experts who reviewed the AIID data and made phase determinations. Please provide: (1) panel composition, (2) methodology used, (3) their phase determinations, (4) comparison with model outputs.}

\subsection{Hidden Markov Model Analysis}
\label{sub:3_hmm_analysis}

We fitted a Gaussian \gls{hmm} with six latent states to identify underlying risk regimes in the AV incident series. The model achieved a log-likelihood of $248.15$ after convergence. Figure~\ref{fig:hmm_states_av} visualizes state assignments over time; Table~\ref{tab:hmm_states} summarizes state characteristics.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/fig8_hmm_states.png}
    \caption{HMM State Assignments for AV Incidents (2014--2025). Points indicate monthly incidents colored by latent state; the bottom strip shows state assignments over time. Blue tones represent low-activity states (77\% of months); orange/red indicates elevated and crisis states. The two Extreme Spike observations correspond to the Tesla and Uber fatality periods.}
    \label{fig:hmm_states_av}
\end{figure}

\begin{table}[htbp]
\centering
\caption{HMM State Characteristics.}
\label{tab:hmm_states}
\small
\begin{tabular}{lrrr}
\toprule
State & Mean & Months & \% \\
\midrule
Baseline & 0.0 & 73 & 57 \\
Low Activity & 1.0 & 26 & 20 \\
Moderate & 1.0 & 12 & 9 \\
Elevated & 2.0 & 2 & 2 \\
High & 2.2 & 13 & 10 \\
Extreme Spike & 4.0 & 2 & 2 \\
\bottomrule
\end{tabular}
\end{table}

The HMM reveals that AV incidents spend 77\% of months in low-activity states (Baseline + Low Activity), with elevated states occurring episodically rather than persistently. The two Extreme Spike months (mean = 4.0) correspond to the Tesla and Uber fatalities, indicating that crisis events generate incident volumes several times above baseline.

\paragraph{Note on Interpretation.} HMM states represent activity \textit{levels} based on incident counts alone. They cannot distinguish whether low activity reflects successful mitigation or simply rare occurrence. Note that with a mean of 0.6 incidents per month, the six-state model is likely over-specified for this sparse data --- Low Activity and Moderate both correspond to months with exactly one incident and are distinguished only by their transition dynamics rather than count magnitude. Section~\ref{sub:3_phase_classification} addresses this limitation by incorporating trend information to produce governance-relevant phase classifications.


\subsection{Changepoint Detection}
\label{sub:3_changepoint_detection}

We applied the \acrfull{pelt} algorithm \cite{killick2012optimal} to identify structural breaks in the AV incident time series. \gls*{pelt} optimizes the detection of multiple \glslink{changepoint_detection}{changepoints} by minimizing a penalized cost function, with the penalty parameter controlling sensitivity to regime changes.

We tested four penalty levels calibrated to the data: Conservative ($3.0 \cdot \log(n) \cdot \sigma^2$), Moderate ($2.0 \cdot \log(n) \cdot \sigma^2$), Sensitive ($1.0 \cdot \log(n) \cdot \sigma^2$), and Exploratory ($0.5 \cdot \log(n) \cdot \sigma^2$). The Exploratory penalty ($\rho = 2.43$) yielded five segments, which we selected for its alignment with known industry events (Figure~\ref{fig:pelt_av}, Table~\ref{tab:pelt_segments}).

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/fig9_pelt_segments.png}
    \caption{\gls*{pelt} Changepoint Detection for Autonomous Vehicle Incidents. \textit{Top panel}: Standardized risk signal with detected changepoints (red dashed lines). \textit{Bottom panel}: Color-coded segments showing distinct incident regimes. The algorithm identifies five segments corresponding to pre-commercial baseline (2014--2017), the crisis period surrounding the Uber ATG fatality (2017--2018), a regulatory pause (2018--2021), post-pause expansion (2021--2022), and scaled commercial deployment (2022--present).}
    \label{fig:pelt_av}
\end{figure}

\begin{table}[htbp]
\centering
\caption{\gls*{pelt}-Detected Segments in AV Incidents (2014--2025)}
\label{tab:pelt_segments}
\begin{tabular}{clcccp{4.2cm}}
\toprule
Seg & Period & Months & $\bar{x}$ & Risk ($\sigma$) & Interpretation \\
\midrule
1 & Jul 2014 -- Oct 2017 & 40 & 0.2 & $-0.42$ & Pre-commercial baseline \\
2 & Nov 2017 -- Aug 2018 & 10 & 1.1 & $+0.55$ & Peak crisis period \\
3 & Sep 2018 -- Feb 2021 & 30 & 0.5 & $-0.17$ & Regulatory pause \\
4 & Mar 2021 -- May 2022 & 15 & 1.3 & $+0.75$ & Post-pause expansion \\
5 & Jun 2022 -- Feb 2025 & 33 & 0.8 & $+0.16$ & Scaled deployment \\
\bottomrule
\end{tabular}
\end{table}

The changepoint analysis reveals a non-monotonic trajectory characterized by distinct crisis and recovery periods. Segment 2 (November 2017 -- August 2018) exhibits the highest mean incident count ($\bar{x} = 1.1$) and risk level ($+0.55\sigma$) among early segments, corresponding to the period surrounding the fatal Uber ATG collision in Tempe, Arizona (March 2018). Notably, this segment shows a strong negative within-segment trend ($\beta = -0.188$), indicating rapid de-escalation following the incident.

The extended Segment 3 (30 months) represents a ``regulatory pause'' during which Uber suspended autonomous operations, multiple states tightened testing requirements, and the industry collectively reduced public road testing. The current Segment 5, spanning nearly three years, shows modest elevation above the historical mean ($+0.16\sigma$) despite substantial increases in deployment scale---suggesting that incident rates per vehicle-mile may actually be declining.

\subsection{Phase Classification}
\label{sub:3_phase_classification}

Applying the classification criteria from Table~\ref{tab:phase_criteria} yields Figure~\ref{fig:phase_timeline_av}. Unlike HMM states, which cluster by count magnitude alone, phase classification combines risk level ($z$-score) with trend direction ($\tau$) to distinguish improving from deteriorating conditions.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/phase_timeline_6_sdcars.png}
    \caption{Phase Classification for AV Incidents (2014--2025). Points indicate monthly incidents colored by governance phase; the bottom strip shows phase assignments over time. The ``striped'' pattern demonstrates that the domain oscillates between baseline and crisis states rather than settling into persistent endemicity.}
    \label{fig:phase_timeline_av}
\end{figure}

Comparing Figures~\ref{fig:hmm_states_av} and \ref{fig:phase_timeline_av} illustrates the distinction: a month with moderate incident counts appears as a single HMM state (e.g., ``Moderate'') but may be classified as either ``Endemic Mitigated'' (if trend is declining) or ``Rapid Expansion'' (if trend is rising). This interpretive layer transforms statistical signal into governance-relevant categories.

Table~\ref{tab:phase_6_av} summarizes the phase distribution. Three patterns merit attention:

\begin{table}[htbp]
\centering
\caption{Phase Distribution for AV Incidents.}
\label{tab:phase_6_av}
\small
\begin{tabular}{lrr}
\toprule
Phase & Months & \% \\
\midrule
No Evidenced Occurrence & 73 & 57 \\
Rare Mitigated & 0 & 0 \\
Rare Occurrence & 0 & 0 \\
Endemic Mitigated & 26 & 20 \\
Rapid Expansion & 16 & 12 \\
Endemic Unmitigated & 13 & 10 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Crisis-Recovery Cycles.} The 2016 Tesla and 2018 Uber fatalities triggered sharp transitions to Rapid Expansion, followed by return to baseline within 6--12 months. This responsiveness reflects the AV industry's exposure to regulatory action, legal liability, and reputational consequences.

\paragraph{No Sustained Endemicity.} Despite a decade of deployment, AV incidents have not stabilized into Endemic Unmitigated status. The domain spends only 10\% of months in this highest-risk phase, compared to 57\% in the No Evidenced Occurrence phase where no incidents were recorded.

\paragraph{Current Status.} The domain is classified as \textbf{Rapid Expansion}, driven by recent deployment scaling (Waymo, Cruise successors). However, the historical pattern suggests the industry retains capacity for phase regression if incidents escalate.

% \subsection{A Meta-Reporting Card for AI Governance}
% \label{sub:3_meta_reporting_card}

% A central purpose of incident reporting is to support actionable governance. Existing analyses often rely on raw counts or trend lines, possibly conflating reporting intensity with underlying risk, which can be the source of ambiguous or misleading signals to policymakers and the public. By contrast, phase determination directly enables precise and differentiated regulatory actions: see Table~\ref{tab:governance_levers} for examples of generic policy responses.

% \begin{table}[ht]
% \centering
% \begin{tabularx}{\textwidth}{l X}
% \toprule
% \textbf{Phase} & \textbf{Governance Levers} \\
% \midrule
% 1. No Evidenced Occurrence & ``Absence of evidence'' is not ``evidence of absence'': governance includes baseline horizon scanning, indicator design, voluntary reporting channels, sandbox-based observation of new systems, and pre-deployment risk and impact assessments. \\[0.4em]
% \midrule
% 2. Rare Occurrence & Targeted monitoring, early-warning systems, sandbox requirements. \\
% \midrule
% 3. Rapid Expansion & Mandatory reporting, pre-market evidence, crisis coordination. \\
% \midrule
% 4. Endemic Unmitigated & Enforcement, audits, mandatory guardrails, post-market surveillance. \\
% \midrule
% 5. Endemic Mitigated & Ongoing post-market surveillance at reduced but regular frequency; periodic recertification or conformity checks; monitoring for capability drift, dataset changes, and new deployment contexts; updated transparency reports and user documentation; evaluation of mitigation effectiveness using severity-adjusted incident rates. \\[0.4em]
% \midrule
% 6. Rare Mitigated & Regular audits to verify that safeguards remain effective; periodic review of mitigation durability and standards; maintained channels for stakeholder and whistleblower reporting. \\
% \bottomrule
% \end{tabularx}
% \caption{Governance Levers Across Phases.}
% \label{tab:governance_levers}
% \end{table}

% As a practical illustration of how the phase model can support governance, we developed a meta-reporting card prototype that summarizes the evolving status of individual AI incident subdomains (see Figure~\ref{fig:meta_reporting_card_v2}). Rather than functioning as an analytical result of the model itself, the card serves as a translation tool that consolidates key indicators into a format that can guide monitoring and decision-making. Each card synthesizes both quantitative signals such as incident frequency, exposure-adjusted rates, and qualitative assessments, including regulatory developments, and the maturity of mitigation measures.

% The card integrates data fields harmonized across the AI Incident Database (AIID) and the MIT AI Risk Repository, enabling a consistent representation of how a given incident type progresses across different phases. By presenting the current phase classification, documenting historical transitions, and outlining the criteria required for reclassification, the prototype establishes a structured mechanism for updating assessments as new evidence becomes available.

% This lifecycle-aware meta-reporting card for autonomous vehicle incidents would allow regulators, safety assessors, and auditors to interpret incident trends in relation to deployment exposure, operational design domain (ODD), and the maturity of safety controls. By structuring reporting around the six phases from ``no evidenced occurrence'' to ``rare mitigated'', the card could eventually contextualize AV incidents relative to miles driven, fleet size, geographical expansion, and regulatory oversight intensity. For AVs, phase transitions often reflect changes in deployment scale (e.g., entry into new cities), system updates, or governance shocks such as permit suspensions and post-incident audits.

% A complete version of the card, based on more exhaustive data (see Section~\ref{sub:5_implications_ai_governance} for suggestions to improve reporting data), would summarize:
% \begin{enumerate}[nolistsep]
% \item the current phase classification and supporting evidence,
% \item the safety controls and monitoring requirements currently in force,
% \item discrepancies between expected and observed incident patterns, and
% \item regulatory signals across jurisdictions (e.g., California DMV crash and disengagement reporting, EU vehicle safety frameworks, and China's intelligent-vehicle pilot regulations).
% \end{enumerate}

% By doing so, the meta-reporting card would transform operational incident data into a structured, decision-relevant signal of whether AV harms are stabilizing, accelerating, or under effective control.

% \begin{figure}[h!]
%     \begin{tcolorbox}[
%         colback=white,
%         colframe=black!70,
%         fonttitle=\bfseries\large,
%         title=Autonomous Vehicle Incidents: Status Report,
%         boxrule=1pt,
%         arc=2pt
%     ]

%     \emph{Disclaimer: This assessment is based on a statistical model applied to inherently noisy and incomplete data. Whilst the model attempts to account for biases, the analysis should be treated as indicative and reviewed by experts before actions are taken.}

%     \begin{center}
%     \colorbox{orange!20}{
%         \parbox{0.9\linewidth}{
%             \centering\vspace{0.3em}
%             {\large\textbf{Current Phase:}} {\LARGE\textcolor{orange!80!black}{\textbf{RAPID EXPANSION}}}\\[0.2em]
%             {\small February 2025 $\cdot$ Confidence: Moderate}
%             \vspace{0.3em}
%         }
%     }
%     \end{center}

%     \vspace{0.5em}

%     \begin{minipage}[t]{0.48\linewidth}
%         \textbf{What This Means}\\[0.3em]
%         {\small
%         Incident counts are \textbf{above average} and \textbf{trending upward}. First sustained elevation since 2018.\\[0.5em]
%         \textit{Likely driver:} Deployment scaling (Waymo, Cruise successors), not deteriorating per-mile safety.
%         }
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.48\linewidth}
%         \textbf{Historical Context}\\[0.3em]
%         {\small
%         \begin{tabular}{lr}
%         No Evidenced Occurrence months & 57\% \\
%         Endemic Mitigated & 20\% \\
%         Endemic Unmitigated & 10\% \\
%         \end{tabular}\\[0.5em]
%         Pattern: Sparse incidents with episodic clusters. Post-2016 and post-2018 peaks returned to baseline.
%         }
%     \end{minipage}

%     \vspace{0.8em}

%     \includegraphics[width=\linewidth]{figures/meta_card_phase_sdcars.png}

%     \vspace{0.5em}

%     \begin{tcolorbox}[
%         colback=blue!5,
%         colframe=blue!40,
%         boxrule=0.5pt,
%         arc=1pt,
%         left=2mm, right=2mm, top=1mm, bottom=1mm
%     ]
%     \textbf{Suggested Actions}\\[0.2em]
%     {\small
%     \textbf{1.} Increase monitoring frequency from quarterly to monthly;\\
%     \textbf{2.} Track exposure-adjusted rates (incidents per million miles);\\
%     \textbf{3.} Flag if elevation persists beyond 6 months (outside historical pattern).
%     }
%     \end{tcolorbox}

%     \vspace{0.5em}

%     {\footnotesize\color{gray}
%     \textbf{Data:} 75 incidents, 565 reports (Jul 2014 -- Feb 2025)\\
%     \textbf{Sources:} AIID + California DMV\\
%     \textbf{Method:} Phase classification (Section~\ref{sub:3_phase_classification})
%     }

%     \end{tcolorbox}
%     \caption{Meta-reporting Card for Autonomous Vehicles. Designed to translate phase analysis into actionable governance guidance.}
%     \label{fig:meta_reporting_card_v2}
% \end{figure}


==> main_document/4_deepfakes.tex <==
\subsection{Data Characteristics and Proxies}
\label{sub:c_data_characteristics}

Unlike autonomous vehicles, which are physical assets operated by regulated entities, deepfakes are digital artifacts created by distributed, often anonymous users. This difference creates noise unless we isolate unique incidents: a single viral deepfake event can generate multiple news reports, creating massive spikes that reflect temporal media attention. We therefore analyzed unique incidents, using each incident's first reported date to track risk over time.

We curated deepfake-related incidents from the AIID using two methods. First, we searched incident summaries for keywords (``deepfake,'' ``voice cloning,'' ``ai-cloned,'' etc.), excluding false positives related to legislative discussions. Second, we included all incidents labeled under ``Deepfake Video Generation'' or ``Voice Generation'' in the dataset taxonomy. The resulting dataset contains 296 unique incidents with 1,114 related reports, spanning March 2017 to September 2025.

Unlike the AV domain, which benefits from California DMV mileage as a direct exposure denominator, deepfakes lack a natural deployment metric. We constructed an exposure proxy from the cumulative GitHub Stars of eight major open-source deepfake repositories (e.g., \textit{FaceSwap},  \textit{DeepFaceLab}, \textit{Roop}, \textit{FaceFusion}), depreciated with a 24-month half-life to approximate the currently active installed base of accessible tools. This proxy is used as a log-offset in the Negative Binomial GLM described below. A sensitivity analysis across half-lives of 6, 12, and 24 months confirms that the binary dormant-to-endemic finding is robust to this choice (Appendix~\ref{sub:c_halflife_sensitivity_df}). Google Trends data for the search term ``deepfake'' (worldwide, monthly) serve as a media visibility covariate. Full construction details are provided in Appendix~\ref{sub:c_media_adj_risk_nb_df}.

Figure~\ref{fig:03_time_series_overview} visualizes the raw temporal distribution. Incidents remained infrequent through 2021, with raw counts surging sharply in 2023. As we show below, the risk-adjusted signal---which controls for media attention and tool availability---identifies the structural break earlier, in March 2022.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{Figures/Fig_DF/03_time_series_overview.png}
    \caption{Raw Temporal Distribution of Deepfake Incidents and Reports (March 2017--September 2025). Both metrics remained infrequent prior to 2023. Beginning in 2023, frequency increased sharply and displayed intermittent spikes. This trajectory differs markedly from patterns observed in the AV case, which exhibits oscillatory crisis-recovery cycles.}
    \label{fig:03_time_series_overview}
\end{figure}

A notable feature of this domain is reporting speed. While incidents before 2019 often had lags of several years (retrospective discovery), the post-2021 period has a median discovery lag of just 1.0 day (mean 17.0 days), suggesting the database captures near-real-time public concern. To address possible delays in recent months, we applied a nowcasting correction based on the observed distribution of reporting lags. This prevents the artificial ``drop-off'' in late 2025, ensuring that observed declines reflect genuine trends rather than incomplete reporting.

To separate risk escalation from media hype, we constructed a \textbf{media-adjusted excess risk} signal using Negative Binomial regression (details in Appendix~\ref{sub:c_media_adj_risk_nb_df}). This signal controls for two confounds: media-driven reporting bias and growing tool availability. The model finds marginally significant quadratic acceleration ($p = 0.055$) and a positive but not statistically significant media amplification effect (rate ratio = 1.88, $p = 0.121$). Neither covariate reaches conventional significance at $\alpha = 0.05$, so the media-adjusted excess risk signal used in  all subsequent analyses should be interpreted as an approximate correction. 

\begin{table}[htbp]
    \centering
    \caption{Model Parameters: Deepfake Incidents}
    \label{tab:df_params}
    \small
    \begin{tabular}{l l l}
    \toprule
    Model & Parameter & Value \\
    \midrule
    
    Delay model 
    & Median lag (post-2021) 
    & 1.0 days \\
    & Nowcast window 
    & 4 months \\
    & Empirical CDF $P(\text{lag} \le 4\text{m})$ 
    & 97.7\% \\
    
    \addlinespace
    
    NB GLM 
    & Log-Likelihood 
    & $-163.48$ \\
    & Time (quadratic) $p$-value 
    & $0.055$ \\
    & Media Index rate ratio 
    & 1.88 ($p = 0.121$) \\
    
    \addlinespace
    
    PELT 
    & Penalty ($\rho$) 
    & 3.00 (plateau stability) \\
    & Segments detected 
    & 3 \\
    
    \addlinespace
    
    K-means (2D: level + trend)
    & $K$ (clusters) 
    & 5 (silhouette = 0.393) \\
    & Macro-bands
    & 2 (Low $\le -0.5\sigma$, High $\ge +0.5\sigma$) \\
    
    \addlinespace
    
    Forecasting ensemble 
    & Models used 
    & ARIMA(1,1,1), Prophet, GPR \\
    & Divergence (Max--Min)/Max
    & 46.7\% \\
    
    \bottomrule
    \multicolumn{3}{p{11cm}}{\footnotesize \textit{Note:} Full model specification and diagnostics are provided in Appendix~\ref{sub:c_media_adj_risk_nb_df}.} 
    \end{tabular}                                           
  \end{table} 

\subsection{Changepoint Detection}
\label{sub:c_changepoint_detection}
To define when risk becomes critical, we applied Statistical Process Control (SPC) to the media-adjusted excess risk signal. We used the extended dormant period (2018--2022) as our baseline to calculate the historical variance ($\sigma$).\footnote{The SPC reference window extends to end-2022 ($<$ January 2023), which includes the first 10 months of PELT Segment~3 (March--December 2022). In a strictly SPC-pure design, the baseline should be limited to ``in-control'' data only (i.e., pre-March 2022). However, this boundary choice does not affect any conclusions: the highest-risk month in Segment~3 reaches only $+0.43\sigma$ (standardized), while the SPC Epidemic Threshold ($+2\sigma$) and Acute Outbreak threshold ($+3\sigma$) remain well above any observed value under either baseline definition. Tightening the baseline to pre-March 2022 shifts $\mu$ by approximately $+0.12\sigma$, which does not alter whether any month is considered to breach the SPC thresholds.} Under standard SPC doctrine, $+2\sigma$ defines the \textit{Epidemic Threshold} and $+3\sigma$ an \textit{Acute Outbreak}.

To identify when the system breached these control limits, we applied the PELT algorithm with a penalty sweep across $\rho \in [0.5, 10.0]$. Rather than selecting the penalty by heuristic, we used a \textit{plateau stability criterion}: we chose the segmentation that persists across the widest range of penalty values (Table~\ref{tab:pelt_segments_df}). The 3-segment solution appears in 10 of 20 penalty values tested ($\rho \in [3.0, 7.5]$), compared to 5 segments (4 appearances in $\rho \in [1.0, 2.5]$). The 5-segment decomposition is reported in Appendix~\ref{sub:c_pelt_sensitivity_df}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{Figures/Fig_DF/09_pelt_adaptive_success.png}
    \caption{PELT Changepoint Detection for Deepfake Incidents. \textit{Top panel}: Standardized excess risk signal with detected changepoints (red dashed lines). \textit{Middle panel}: Color-coded segments showing distinct reporting regimes. The algorithm identifies a clear structural break in March 2022, marking the transition from a dormant regime to a sustained high-risk state. \textit{Bottom panel:} Segment statistics.}
    \label{fig:pelt_df}
\end{figure}

\begin{table}[htbp]
    \centering
    \caption{PELT-Detected Segments in Deepfake Incident Reporting (2017--2025)}
    \label{tab:pelt_segments_df}
    \small
    \begin{tabular}{c l c c c l}
    \toprule
    Seg & Period & Months & Risk ($\sigma$) & Slope & Interpretation \\
    \midrule
    1 & Mar 2017 -- Jun 2020 & 40 & $-0.05$ & $+0.005$ & Pre-commercial baseline \\
    2 & Jul 2020 -- Feb 2022 & 20 & $-0.83$ & $+0.027$ & COVID-era trough \\
    3 & Mar 2022 -- Sep 2025 & 43 & $+0.43$ & $-0.009$ & \textbf{Endemic plateau} \\
    \bottomrule
    \end{tabular}
\end{table}

The analysis reveals a different pattern from the AV case. Deepfake risk shows a one-way jump. Segments~1--2 (March 2017 to February 2022) form a prolonged incubation period with risk well below the historical mean. The critical rupture occurs in Segment~3 (March 2022 onward), where risk surged to $+0.43\sigma$ and persisted for 43 consecutive months, coinciding with the mainstream release of high-fidelity generative AI tools (\textit{Roop}, \textit{FaceFusion}). A supplementary 5-segment decomposition (Appendix~\ref{sub:c_pelt_sensitivity_df}) reveals sub-structure within this regime, including a sharp 2023 shock (risk $= +0.69\sigma$) followed by a late-period decline, but these sub-phases do not change the binary dormant-to-endemic finding.

Unlike the AV Segment (November 2017 to August 2018) that showed strong within-segment de-escalation that reflecting Uber's operational suspension, the deepfake Segment~3 exhibits a near-flat slope ($-0.009$), showing a structural regime shift.



\subsection{Epidemiological Phase Classification}
\label{subsec:phase_class_df}

Building on the PELT segmentation and K-Means consistency check (Appendix~\ref{sec:c_deepfakes}), we classified each PELT segment into one of three epidemiological phases based on its mean risk level and slope. We set the phase threshold using the pre-2022 reference period (Segments~1--2) as a baseline distribution. The threshold $\theta_{\text{low}} = +0.14\sigma$ equals the upper 1-standard-deviation bound of this baseline ($\mu_d + \sigma_d$, where $\mu_d = -0.26\sigma$ and $\sigma_d = 0.40\sigma$). Values above this threshold represent a statistically unusual departure from baseline. A sensitivity sweep confirms that the binary dormant-to-endemic classification is stable across $\theta \in (-0.05\sigma, +0.43\sigma)$ (Appendix~\ref{sub:c_pelt_sensitivity_df}).

\begin{enumerate}
    \item \textbf{Dormant Baseline} (Risk $< +0.14\sigma$): The historical incubation period where incidents remained constrained to early technical demonstrations or localized misuse. Corresponds to PELT Segments~1--2 and the low-risk K-Means macro-band.
    \item \textbf{Active Outbreak} (Risk $\ge +2\sigma$ \textit{or} Slope $> \tau_{\text{rapid}}$): Months exhibiting explosive growth or actively breaching the SPC Epidemic Threshold. The slope threshold $\tau_{\text{rapid}} = \max(\text{P}_{75}(\text{slopes}), 0.05)$ per month is calibrated to the observed segment distribution; for this dataset $\tau_{\text{rapid}} = 0.05$, matching the fixed value used in sensitivity analyses.
    \item \textbf{Endemic Unmitigated} (Risk $\ge +0.14\sigma$, not meeting Outbreak criteria): The elevated stabilization state where risk persists structurally above the dormant reference distribution but has ceased rapid escalation. Corresponds to PELT Segment~3 and the high-risk K-Means macro-band.
\end{enumerate}

The resulting phase distribution across the 103-month observation window is:

\begin{table}[htbp]
    \centering
    \caption{Phase Distribution for Deepfake Incidents (2017--2025).}
    \label{tab:phase_dist_df}
    \small
    \begin{tabular}{lrr}
    \toprule
    Phase & Months & \% \\
    \midrule
    Dormant Baseline & 60 & 58.3 \\
    Active Outbreak & 0 & 0.0 \\
    Endemic Unmitigated & 43 & 41.7 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/Fig_DF/12_phase_timeline_deepfake.png}
    \caption{Deepfake incident timeline with model-derived phase classification (2017--2025). Annotated events mark incident spikes alongside landmark repository releases (Roop, FaceFusion). The horizontal strip visualizes phase transitions over time.}
    \label{fig:phase_dist_df}
\end{figure}

To verify consistency with the AV methodology, we applied the full six-phase classification framework (Table~\ref{tab:phase_criteria}) to the primary 3-segment PELT model. Of six possible phases, only two are populated: \textit{No Evidenced Occurrence} (58.3\%) and \textit{Endemic Mitigated} (41.7\%). The remaining four phases are never occupied, confirming that the deepfake domain lacks the oscillatory dynamics that populate four of six phases in the AV domain (full details in Appendix~\ref{sub:c_pelt_sensitivity_df}). The 5-segment sensitivity model populates three 6-phase labels (adding Rare Mitigated for the Oct 2021--Dec 2022 transitional segment), but confirms the same binary conclusion: all pre-2022 months fall into low-risk phases, and the post-2023 period is the sole elevated-risk epoch.                                                       
                                                   
A clarification on labeling: the six-phase system classifies Segment~3 as \textit{Endemic Mitigated} because its risk ($+0.43\sigma$) falls between $\theta_{\text{low}}$ and $\theta_{\text{high}}$ with a declining slope, whereas the simplified three-phase system used throughout this section classifies it as \textit{Endemic Unmitigated} because any risk above $\theta_{\text{low}}$ qualifies. The meta-reporting card (Figure~\ref{Figures/Fig_DF/12_phase_timeline_deepfake.png}) follows the three-phase convention. Both systems agree that Segment~3 represents a structurally elevated endemic regime; they differ only on whether the modest within-segment decline constitutes evidence of mitigation. We adopt the more conservative three-phase label (\textit{Endemic Unmitigated}) for the primary analysis because no external intervention has been shown to reduce deepfake risk (Section~\ref{sub:c_df_limitations}).

Two features of the simplified distribution merit emphasis. First, the absence of months classified as Active Outbreak (0\%) is a substantive finding. Unlike the AV domain, where the 2018 Uber fatality generated a brief but unmistakable spike, the deepfake trajectory never exhibits a single-month catastrophic breach. Instead, the risk signal climbed above baseline and stayed there, \textit{bypassing} the Outbreak phase entirely and settling directly into Endemic status---a 43-month plateau at $+0.43\sigma$ (Segment~3).

Second, the 58.3\% Dormant classification reflects a long pre-2022 incubation period (Segments~1--2). The deepfake domain spent nearly five years in dormancy in the dataset before transitioning into endemicity in March 2022. This contrasts with the AV domain, reflecting the industry's persistent capacity for phase regression after crisis events.

The contrast between physical (AV) and digital (Deepfake) risk trajectories lies in what we term the ``Endemic Trap.'' In the AV case, the 2018 Uber fatality triggered Uber's immediate suspension of all autonomous operations, regulatory investigations across multiple states, and a sector-wide de-escalation. The system \textit{recovered} to baseline within 12 months. This response is possible because AV deployment is centralized: a small number of corporations operate identifiable fleets under government permits.

Deepfakes are generated by distributed users downloading open-source tools from public repositories. No single corporate actor controls the technology, and no regulatory body can issue a ``recall'' on software that has already been forked thousands of times on GitHub. Consequently, once the deepfake trajectory entered the Endemic phase in March 2022, the system remained there for 43 consecutive months with no structural recovery.






\subsection{Methodological Limitations and Threats to Validity}
\label{sub:c_df_limitations}

While PELT and SPC provide a rigorous framework for analyzing deepfake risk, the reliance on crowdsourced databases introduces structural limitations:

\begin{enumerate}
    \item \textbf{Selection Bias and the ``Hype Cycle'' Confound}: The AI Incident Database relies on voluntary reporting and journalistic discovery. Consequently, the observed incident surge in 2023 is inextricably linked to the intense global media attention surrounding generative AI. Although our Negative Binomial regression framework explicitly controls for public attention using a normalized Google Trends media index, no empirical adjustment can perfectly disentangle the true proliferation of risk from the heightened vigilance of database contributors searching for deepfake incidents during an AI hype cycle. 
    
    \item \textbf{Left-Censorship of the Baseline}: The period from 2018 to 2022 serves as the historical baseline for calculating the SPC epidemic control limits ($\pm 2\sigma$). However, prior to 2023, the majority of deepfake misuses involved localized deployment scattered across underground forums. Because early incidents received less mainstream news coverage than recent political and financial disruptions, they are underrepresented in the dataset. This ``left-censorship'' artificially depresses the historical variance ($\sigma$). Thus, the magnitude of the control limit breach during the ``2023 Shock'' may be partially inflated by the artificial suppression of the historical baseline.

    \item \textbf{Qualitative Compression and Severity Agnosticism}: To enable objective mathematical time-series modeling, our incident-centric pipeline implicitly assigns equal statistical weight to all registered incidents. An early academic demonstration video is mathematically indistinguishable from a coordinated multi-million dollar international fraud campaign. Therefore, our definition of an ``Epidemic'' phase captures a strictly \textit{quantitative} shift in incident frequency, and does not differentiate based on the qualitative severity of societal harm.
    \item \textbf{Right-Censoring of the Reporting Tail}: Incident databases such as AIID exhibit systematic right-censoring: incidents from the most recent months are underrepresented because the full cycle of occurrence, discovery, reporting, and editorial curation has not yet completed. For the deepfake corpus, the post-2021 empirical lag distribution has a median of 0 months and a 95th percentile of 4 months, so the pipeline applies an empirical CDF nowcasting correction to the final 4-month window (inflating raw counts by up to 5$\times$ for the most recent month). This hard cap prevents implausible corrections for months with very few observations but introduces a conservative bias: if the true reporting delay distribution has a longer right tail, the capped correction will undercount recent incidents.

    This correction addresses the level of incident counts but does not fully eliminate the risk of \textit{false phase regression}: a brief tail of artificially low nowcasted counts could, in principle, trigger a spurious PELT changepoint near the analysis endpoint and cause a short recent segment to be misclassified into a lower-risk phase. The primary structural safeguard is that PELT computes phase labels from \textit{segment means}, not individual monthly values; Segment~3 spans 43 months, so the 4-month nowcast tail carries less than 10\% weight in the mean, making the current \textit{Endemic Unmitigated} classification robust to right-censoring. For the present snapshot analysis (endpoint September 2025), Segment~3 mean risk of $+0.43\sigma$ comfortably exceeds the $+0.14\sigma$ Endemic threshold even after removing the final 4 months. This caveat becomes more material in a live streaming deployment, where a minimum-duration confirmation window (requiring a declining trend to persist for a specified number of months before accepting a phase downgrade) would be a prudent additional safeguard.
\end{enumerate}

Despite these limitations, the persistence of the high-risk Endemic plateau across sensitivity sweeps shows that the post-2022 phase transition represents a structural shift in the socio-technical ecosystem, rather than observational noise.






% smylius@gmail.com
% \begin{tcolorbox}[
%     title=Meta-Reporting Card Prototype for Deepfake-Enabled Incidents,
%     colback=gray!5,
%     colframe=black,
%     fonttitle=\bfseries
% ]
% \emph{Disclaimer: This assessment is based on a statistical model applied to inherently noisy and incomplete data. Whilst the model attempts to account for biases, the analysis should be treated as indicative and reviewed by experts before actions are taken.}\\

% \textbf{Key Indicators}:
% \begin{itemize}[nolistsep]
%     \item 296 AIID Incidents;
%     \item 1,114 Individual Reports;
%     \item Date Range: March 2017 to September 2025;
%     \item Exposure data: Google Trends and GitHub stars (8 major deepfake repositories)
% \end{itemize}
% \textbf{Current Status (October 2025)}: \textcolor{red}{\textbf{Endemic Unmitigated}}\footnote{Despite a slight decline in the most recent months, the phase remains classified as Endemic Unmitigated due to lag protection. Segments showing declining trends are only reclassified as ``Mitigated'' if the decline has persisted for more than 3 months from the analysis date. This buffer prevents premature recovery signals caused by incomplete reporting or transient fluctuations.}\\
% \textbf{Confidence}: High.\\
% \textbf{Actionable Policy Recommendation}:
% \begin{itemize}[nolistsep]
%     \item Restrict access rate to providers of AI systems capable of generating highly-realistic deepfakes;
%     \item Enforce stricter control on platforms enabling large-scale propagation of generated content (e.g., social media).
% \end{itemize}
% \includegraphics[width=\linewidth]{Figures/Fig_DF/12_meta_card_phase_deepfake.png}
% \textbf{Key Insights}:
% \begin{itemize}[nolistsep]
%     \item Quadratic acceleration of risk pattern starting from 2023;
%     \item Irreversible phase transition triggered by a stark increase in generative video/voice tools;
% \end{itemize}
% \textbf{Notable Incident Periods}:
% \begin{itemize}[nolistsep]
%     \item "2023 Shock" (Jan 2023--May 2023)
% \end{itemize}
% \textbf{Main MIT Incident Type}: 
% \begin{itemize}[nolistsep]
%     \item   4.3 Fraud, scams, and targeted manipulation (184 / 296)
%     \item   4.1 Disinformation, surveillance, and influence at scale (70 / 296)
%     \item   3.1 False or misleading information (32 / 296).
% \end{itemize}
% \end{tcolorbox}

% \begin{figure}[h!]
%     \begin{tcolorbox}[
%         colback=white,
%         colframe=black!70,
%         fonttitle=\bfseries\large,
%         title=Deepfake Incidents: Status Report,
%         boxrule=1pt,
%         arc=2pt
%     ]
    
%     \emph{Disclaimer: This assessment is based on a statistical model applied to inherently noisy and incomplete data. While the model attempts to account for biases, the analysis should be treated as indicative and reviewed by experts before actions are taken.}
    
%     \begin{center}
%     \colorbox{red!20}{
%         \parbox{0.9\linewidth}{
%             \centering\vspace{0.3em}
%             {\large\textbf{Current Phase:}} {\LARGE\textcolor{red!80!black}{\textbf{ENDEMIC UNMITIGATED}}}\\[0.2em]
%             {\small October 2025 $\cdot$ Confidence: Moderate}
%             \vspace{0.3em}
%         }
%     }
%     \end{center}
    
%     \vspace{0.5em}
    
%     \begin{minipage}[t]{0.48\linewidth}
%         \textbf{What This Means}\\[0.3em]
%         {\small 
%          Irreversible phase transition triggered by a stark increase in generative video/voice tools.\\
         
%          Policy interventions have mostly failed to account for the technology adoption.
%         }
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.48\linewidth}
%         \textbf{Historical Context}\\[0.3em]
%         {\small
%         \begin{tabular}{lr}
%         Dormant Baseline & 58.3\% \\
%         Active Outbreak & 0.0\% \\
%         Endemic Unmitigated & 41.7\% \\
%         \end{tabular}\\[0.5em]
%         Pattern: Irreversible step-function transition after the 2022 GenAI shock. No oscillatory recovery.
%         }
%     \end{minipage}
    
%     \vspace{0.8em}
    
%     \includegraphics[width=\linewidth]{Figures/Fig_DF/12_meta_card_phase_deepfake.png}
    
%     \vspace{0.5em}
   
%     \begin{tcolorbox}[
%         colback=blue!5,
%         colframe=blue!40,
%         boxrule=0.5pt,
%         arc=1pt,
%         left=2mm, right=2mm, top=1mm, bottom=1mm
%     ]
%     \textbf{Suggested Actions}\\[0.2em]
%     {\small
%     \textbf{1.} Restrict access rate to providers of AI systems capable of generating highly-realistic deepfakes;
%     \textbf{2.} Enforce stricter control on platforms enabling large-scale propagation of generated content (e.g., social media).
%     }
%     \end{tcolorbox}
    
%     \vspace{0.5em}
    
%     {\footnotesize\color{gray}
%     \textbf{Data:} 296 incidents, 1,114 reports (Mar 2017 -- Sep 2025)\\
%     \textbf{Sources:} AIID + Github Stars\\
%     \textbf{Method:} Phase classification (Section~\ref{subsec:phase_class_df})\\
%     % \textit{Caveat:} Analysis reflects reporting patterns, not ground-truth risk. 
%     }
    
%     \end{tcolorbox}
%     \caption{Meta-Reporting Card for Deepfakes.}
%     \label{fig:meta_reporting_card_df_v2}
% \end{figure}


% Much like for AVs, the meta-reporting card for deepfake-enabled incidents (Figure~\ref{fig:meta_reporting_card_df_v2}) would help regulators, platforms, and auditors interpret fragmented incident data without overreacting to noise or missing early escalation signals. In that case, the card could eventually contextualize each deepfake harm type relative to its exposure, observability, and maturity of governance controls. For deepfakes, this means distinguishing sporadic harms (such as isolated non-consensual sexual images) from phase transitions, including rapid expansion in election interference or a stable endemic level of fraud. 




\noindent\rule{8cm}{0.4pt}

BELOW NOT MIGRATED




==> main_document/6_conclusion.tex <==
ABOVE MIGRATED

\noindent\rule{8cm}{0.4pt}

BELOW NOT MIGRATED

By reframing classes of AI incidents through a lifecycle lens, this paper offers a conceptual and statistical structure that strengthens and complements existing governance tools. Instead of treating raw incident counts as indicators of worsening or improving safety, a phase-based approach provides a more robust, interpretable, and policy-aligned way to understand how harms emerge, escalate, stabilize, or decline and when specific interventions are warranted. 

AI incidents are not isolated failures; they progress through identifiable phases. Recognizing these phases allows governments to detect early warning signals, allocate resources efficiently, and evaluate progress toward safer AI systems. Crucially, our findings emphasize that phase classification is not a purely mechanical output of statistical modeling. It requires interpretation grounded in the operational context of each AI system class, including its deployment environment, exposure profile, and documentation pathways. Below we outline priority directions that would substantially improve the accuracy, usefulness, and fairness of phase-based monitoring.

\subsection{Implications for AI Governance}
\label{sub:5_implications_ai_governance}

The transition from a passive database of incidents to an active phase monitoring system carries three primary implications for governance strategy.

\subsubsection*{For Incident Reporting: Strengthening the Infrastructure and Improving Data Granularity}

Mandating standardized disclosure can be a first step towards facilitating a consistent data collection of AI incidents \citep{dixon2025ai, longpre2025inhouse}. An expansion of the EU AI Act Article 73, warranting reporting to all types of incidents, ideally classified with respect to a common taxonomy (e.g., the MIT Risk Repository's taxonomy \citep{slattery2024ai}, combined with an AI harm taxonomy \citep{hoffman2023adding}), would be a sensible path forward. It would need clear triggers (e.g., "any unintended harm to legal rights"), as well as safe harbor provisions to encourage disclosure. In particular, it may be desirable to incentivize voluntary reporting, e.g., through offering liability protections or regulatory "good faith" credits for firms that disclose near-misses. Also, since most of the reporting effort is being performed by voluntary initiatives, policymakers could support third-party incident databases (e.g., the AIID \citep{mcgregor2021preventing}) to cross-validate industry reports, and fill gaps in understudied sectors (e.g., AI in agriculture, climate modeling).

In addition to improving the incident reporting frameworks as a whole, it may be useful to improve the quality of the incident reports themselves. As mentioned earlier, policymakers should endeavor to standardize incident taxonomies to enable global consistency and interoperability of reporting data \citet{perset2025framework}. Furthermore, for its phase transition identification capabilities to be optimal, our phase model requires real-time or near-real-time reporting incidents. Thus, we suggest policymakers to implement time constraints for mandatory reporting, which could be adapted to the severity of the incident (e.g., in a range from within 24 hours for the most severe incidents, and to within 15 days for the most benign). Finally, it could be useful for more fine-grained analysis to link incident data to deployment context: reporting efforts could collect metadata on system characteristics (e.g., model size, training data sources) and governance environment (e.g., whether the system was audited pre-deployment) \citep{dixon2025ai}. This would allow policymakers to better correlate phases with regulatory interventions.

\subsubsection*{For Policymakers: Resource Allocation and Addressing Structural Biases}

As policymakers operate under resource constraints, our phase model could serve as a triage mechanism: incident types classified as \emph{No Evidenced Occurrence} or \emph{Rare Occurence} may require only passive horizon scanning, while incident types classified as \emph{Rapid Expansion} or \emph{Endemic Unmitigated} warrant immediate investigative resources for risk prevention or damage control. This would allow government agencies to pivot from "policing everything" to "policing the instability."

Furthermore, to ensure global equity in AI incident reporting, it is crucial to establish regional AI safety hubs that would train local incident investigators and provide anonymous reporting channels to protect whistleblowers, taking inspiration from similar endeavors for AI ethics in Africa \citep{adams2025final}.

Finally, policymakers would do well to counteract media-driven distortions through the development of automated tools for the flagging of overrepresented incidents (e.g., viral but low-severity cases) \citep{hamborg2019automated}.


\subsection{Research Directions for Future Work}
\label{sub:5_future_work}

\subsubsection*{Methodological Development}
\begin{itemize}
    \item \textbf{Benchmark Alternative Generative Models.} Evaluate Hawkes processes, Bayesian structural time series, and self-exciting spatial–temporal models on both observed and simulated incident data to identify cases where each approach is most reliable.
    \item \textbf{Improve Nowcasting with Non-Stationary Delays.} Develop delay models that allow time-varying delay distributions (e.g., via covariates or hierarchical models) to better handle editorial changes or regulatory effects on reporting lag.
    \item \textbf{Probabilistic Exposure Models.} Replace deterministic synthetic exposure proxies with probabilistic exposure estimators that propagate uncertainty into phase assignments.
    \item \textbf{Decision-Theoretic Trigger Design.} Formalize trigger thresholds using decision-theory frameworks that balance the social cost of false positives and false negatives for different audiences (e.g., regulators vs. civil-society responders).
    \item \textbf{Incident Classification Framework.} Develop a systematic approach to characterize incident classes by theme to inform selection of classes for modeling.
\end{itemize}

\subsubsection*{Applied and Participatory Work}
\begin{itemize}
    \item \textbf{Co-Design Meta-Reporting Cards.} Pilot co-design workshops with regulators, CSOs, and industry to refine the card’s fields, update cadence, and thresholds for action.
    \item \textbf{Cross-Validation with Administrative Data.} Collaborate with industry and regulators to validate phase assignments against privileged administrative records (e.g., internal incident tracking, verified claims settlements, or audit outcomes).
    \item \textbf{Longitudinal Intervention Studies.} Use phase assignments to identify domains for prospective intervention trials (e.g., mandated guardrails) and to evaluate their effectiveness through quasi-experimental designs.
\end{itemize}

\subsection{Closing Note}
Implementing these research priorities requires both technical work and institutional commitment to better data collection and sharing. The phase-model framework we present is operational today with publicly available data and provides limited governance value; its full potential-accurate, timely, and globally representative monitoring of AI harms-depends on improved exposure reporting, richer incident timestamps, and collaborative partnerships between researchers, civil society, developers, and regulators.

A natural next step is to align the phase model within regulatory regimes that already mandate or anticipate serious-incident reporting. Under the EU AI Act, providers of high-risk and general-purpose AI systems will be required to notify regulators of serious incidents and undertake post-market monitoring; phase classification could serve as an organizing layer for these reports, indicating when a given harm type has moved from rare emergence to rapid expansion or endemic unmitigated status, and therefore warrants tighter supervision, targeted audits, or code-of-practice updates. Likewise, emerging California transparency and incident-reporting laws (e.g.\ around safety incidents in automated systems and AI services) could use phase labels as a way to prioritize enforcement and public disclosure, and to escalate reporting expectations and oversight if an incident class crosses predefined phase thresholds. 

In both contexts, future work should explore how to map legal triggers (e.g.\ ``serious incident'', ``systemic risk'',” or ``material change in risk profile'') onto phase transitions, so that regulators can use a common lifecycle vocabulary to interpret noisy incident data, coordinate responses across jurisdictions, and evaluate whether new rules actually shift specific harms from endemic unmitigated to rare and mitigated states.
